Synthesizing Correlated Randomness using Algebraic Structured Codes

In this problem, Alice and Bob, are provided $X_{1}^{n}$ and $X_{2}^{n}$ that are IID $p_{X_1 X_2}$. Alice and Bob can communicate to Charles over (noiseless) links of rate $R_1$ and $R_2$, respectively. Their goal is to enable Charles generate samples $Y^{n}$ such that the triple $(X_{1}^{n},X_{2}^{n},Y^{n})$ has a PMF that is close, in total variation, to $\prod p_{X_1 X_2 Y}$. In addition, the three parties may posses shared common randomness at rate $C$. We address the problem of characterizing the set of rate triples $(R_1,R_2,C)$ for which the above goal can be accomplished. We build on our recent findings and propose a new coding scheme based on coset codes. We analyze its information-theoretic performance and derive a new inner bound. We identify examples for which the derived inner bound is analytically proven to contain rate triples that are not achievable via any known unstructured code based coding techniques. Our findings build on a variant of soft-covering which generalizes its applicability to the algebraic structured code ensembles. This adds to the advancement of the use structured codes in network information theory.

==> Lemmas.tex <==
\begin{lemma}
\label{Lem:PMFWHP}
% \begin{align}
%   \sum_{l =1}^{2^{n\tilde{R}}} E^{(\mu_1)}_{L|X^n}(l|x^n) \leq 1  \text{ with high probability. } \nonumber
% \end{align}
% $\sum_{l =1}^{2^{n\tilde{R}}} E^{(\mu_1)}_{L|X^n}(l|x^n) \leq 1 $ with high probability if $\tilde{R} \geq I(X;W) + 4\delta$, for all $\delta,\eta \in (0,1)$ and $x^n \in T_{\delta}(X)$.
For any $\delta,\eta \in (0,1),$ if $\tilde{R} > I(X:W)+4\delta$, then
\begin{align}
\PP\left[\bigcap_{\mu=1}^{2^{nC}}\bigcap_{x^n\in T_{\delta}(X)}\left\{E^{(\mu_1)}_{L|X^n}(l|x^n) \leq 1\right\}\right]  \rightarrow 1 \text{ as } n \rightarrow \infty
\end{align}
\end{lemma}
\begin{proof}
From the definition of $E^{(\mu_1)}_{L|X^n}(l|x^n)$, we have \text{ for } $x^n \in T_{\delta}(X), $
\begin{align*}
%   \sum_{l =1}^{2^{n\tilde{R}}}& E^{(\mu_1)}_{L|X^n}(l|x^n) \nonumber \\ 
   \sum_{l =1}^{2^{n\tilde{R}}} E^{(\mu_1)}_{L|X^n}(l|x^n) =  &\frac{1}{2^{n\tilde{R}}} \left(\cfrac{1-\epsilon}{1+\eta}\right) \sum_{\substack{w^n \in \\T_{\delta}(W|x^n)}} \sum_{l=1}^{2^{n\tilde{R}}} \mathbbm{1}_{\{\mathtt{w}^n(l,\mu_1) = w^n\}} \cfrac{p^n_{X|W}(x^n|w^n)}{p^n_X(x^n)} .
\end{align*}
% Since  $x^n \in T_{\delta}(X)$, and the summation is over $w^n \in T_{\delta}(W|x^n)$, we have $Q^n_{X|W}(x^n|w^n) \leq $

Let us define $Z^{(\mu_1)}_l(x^n)$, for $x^n \in T_{\delta}(X)$ as 
\begin{align}\label{def:ZtZ}
    Z_l^{(\mu_1)}(x^n) & = \sum_{w^n \in 
T_{\delta}(W|x^n)}\mathbbm{1}_{\{\mathtt{w}^n(l,\mu_1) = w^n\}} p^n_{X|W}(x^n|w^n) 
(1-\epsilon)
\end{align}
and let $D = 2^{n(H(X|W)-\delta_1)}$, where $\delta_1(\delta) \searrow 0$ as $\delta \searrow 0$. This gives us the following bound on the expectation of the empirical average of $\{Z^{(\mu_1)}_l(x^n)\}_{l \in [2^{n\tilde{R}}]}$ as 
\begin{align}
\label{eq:con1}
    \EE&\bigg[\cfrac{1}{N}\sum_{l=1}^N D Z^{(\mu_1)}_l(x^n) \bigg] \nonumber \\ & = 
2^{n(H(X|W)-\delta_1)} \sum_{w^n \in T_{\delta}(W|x^n)}\tilde{p}_W^n(w^n) 
p^n_{X|W}(x^n|w^n) (1-\epsilon) \nonumber \\
    & \geq 2^{n(H(X|W)-\delta_1)} 2^{-n(H(X,W)+2\delta_1)} 2^{n(H(W|X)-\delta_1)} \nonumber \\
    & \geq 2^{-n(I(X,W)+4\delta_1)}
\end{align}

where in the above equations we use the fact that $\EE[\mathbbm{1}_{\{W^n(l,\mu_1) = w^n\}}] = 
\tilde{P}_W^n(w^n)$.

Further, we also have
\begin{align} \label{eq:con2}
    D Z^{(\mu_1)}_l(x^n) & \leq  2^{n(H(X|W)-\delta_1)} 2^{-n(H(X|W)-\delta_1)}(1-\epsilon)\!\!\!\sum_{w^n \in T_{\delta}(W|x^n)}\mathbbm{1}_{\{W^n(l,\mu_1) = w^n\}}   \leq   1 
\end{align}
where we have bounded $\displaystyle\sum_{w^n \in T_{\delta}(W|x^n)}\mathbbm{1}_{\{W^n(l,\mu_1) = w^n\}}$ by $1$.
% if $x^n \in T_{\delta}(X)$ and $w^n \in T_{\delta}(W|x^n)$ then $(x^n,w^n) \in T_{2\delta}(X,W)$ and $w^n \in T_{\delta_1}(W)$, where $\delta_1= 2|\mathcal{X}|\delta$.

Since $\{Z^{(\mu_1)}_l(x^n)\}_{l}$ is a sequence of IID Random variables, we can approximate its empirical average, for $x^n \in T_{\delta}(X)$, using a more refined Chernoff-Hoeffding bound given by
% \footnote{The Statement of the bound used and its proof is provided in \cite{arxiv_CurrentPaper}}
% to obtain

% \begin{lemma} \label{lem:chernoff}
% Let $\{Z_n\}_{n=1}^N$ be a sequence of N IID random variables bounded between $[0,1]$, such that $\EE\bigg[\cfrac{1}{N}\sum_{n=1}^{N}Z_n\bigg] = \mu  \geq \theta$ where $\theta \in (0,1)$ then
% \begin{align}
%     \PP\bigg(\cfrac{1}{N}\sum_{n=1}^{N}Z_n \in & [(1-\eta)\mu,(1+\eta)\mu] \bigg)  \geq 1 - 2\exp{\bigg(-\cfrac{N\eta^2 \theta}{4 \ln{2}}\bigg)}
% \end{align}
% \end{lemma}
\begin{lemma} \label{lem:chernoff}
Let $\{Z_n\}_{n=1}^N$ be a sequence of N IID random variables bounded between zero and one, i.e., $ Z_n \in [0,1] \quad \forall n \in [N]$, and suppose $\EE\bigg[\cfrac{1}{N}\sum_{n=1}^{N}Z_n\bigg] = \mu$ be lower bounded by a positive constant $\theta$ as $ \mu \geq \theta$ where $\theta \in (0,1)$, then for every $\eta \in (0,1/2)$ and $(1+\eta)\theta < 1$, we can bound the probability that the ensemble average of the sequence $\{Z_n\}_{n=1}^{N}$ lies in $(1\pm \eta)\mu$ as
\begin{align}
    \PP\bigg(\cfrac{1}{N}\sum_{n=1}^{N}Z_n \in & [(1-\eta)\mu,(1+\eta)\mu] \bigg)  \geq 1 - 2\exp{\bigg(-\cfrac{N\eta^2 \theta}{4 \ln{2}}\bigg)}
\end{align}
\end{lemma}
\begin{proof}
Follows from Operator Chernoff Bound \cite{ahlswede2002strong}.
\end{proof}

Note that $\{DZ^{(\mu_1)}_l(x^n)\}_{l}$ satisfies the  constraints from the above lemma from Eqns.  (\ref{eq:con1} and \ref{eq:con2}).
Thus applying Lemma (\ref{lem:chernoff}) to $\{DZ^{(\mu_1)}_l(x^n)\}_{l}$ for every $x^n \in T_{\delta}(X)$ gives
% \begin{lem}{Chernoff Bound} \label{lem:chernoff}
% Let $\{Z_n\}_{n=1}^N$ be a sequence of N IID random variables bounded between $[0,1]$, such that $\EE\bigg[\cfrac{1}{N}\sum_{n=1}^{N}Z_n\bigg] = \mu  \geq \theta$ where $\theta \in (0,1)$ then
% \begin{align}
%     \PP\bigg(\cfrac{1}{N}\sum_{n=1}^{N}Z_n \in [(1-\eta)\mu,(1+\eta)\mu] \bigg) \geq 1 - 2\exp{\bigg(-\cfrac{N\eta^2 a}{4 \ln{2}}\bigg)}
% \end{align}
% \end{lem}
% \begin{proof}
% Follows from Operator Chernoff Bound
% \end{proof}
% Note that $\{DZ^{(\mu_1)}_l(x^n)\}_{l}$ satisfies the Applying the constraints from the above lemma from Eqns.  (\ref{eq:con1} and \ref{eq:con2}).
% Thus applying Lemma (\ref{lem:chernoff}) to $\{DZ^{(\mu_1)}_l(x^n)\}_{l}$ for some $x^n \in T_{\delta}(X)$ gives
\begin{align}\label{eq:chernoff1_Z}
    \!\!\!\!\PP\left( \cfrac{1}{2^{n\tilde{R}}}\sum_{l=1}^{2^{n\tilde{R}}} Z^{(\mu_1)}_l(x^n) \in [(1-\eta)\EE\left[ Z(x^n)\right],(1+\eta)\EE\left[ Z(x^n)\right]]\right) \geq 1 - 2\exp{\bigg(-\cfrac{\eta^2 2^{n(\tilde{R} - I(X,W)-4\delta_1)} }{4 \ln{2}}\bigg)} 
\end{align}
% where we have used the additivity of expectation to simplify $\EE\bigg[\cfrac{1}{N}\sum_{l=1}^N Z^{(\mu_1)}_l(x^n) \bigg]$ and $Z(x^n)$ is used to denote a generic random variable from the IID sequence.
where $Z(x^n)$  denotes the ensemble mean of the IID sequence $\{Z^{(\mu_1)}_l(x^n)\}_{l}$.
Substituting the following simplification
\begin{align}
 \cfrac{1}{2^{n\tilde{R}}}\sum_{l =1}^{2^{n\tilde{R}}}Z_l^{(\mu_1)}(x^n) = (1+\eta)p_{X}^n(x^n) \sum_{l =1}^{2^{n\tilde{R}}}  E^{(\mu_1)}_{L|X^n}(l|x^n) 
\end{align} 
which follows from the definition of $Z_l^n(x^n)$  in (\ref{eq:chernoff1_Z}) gives
\begin{align}
    \PP\left((1+\eta)p_{X}^n(x^n) \sum_{l =1}^{2^{n\tilde{R}}}  E^{(\mu_1)}_{L|X^n}(l|x^n) \leq (1+\eta)\EE{[Z(x^n)]}\right)  \geq 1 - 2\exp{\bigg(-\cfrac{\eta^2 2^{n(\tilde{R} - I(X,W)-4\delta_1)} }{4 \ln{2}}\bigg)} 
\end{align}
Further we can bound $\EE[Z(x^n)]$ as
\begin{align}
    \frac{\EE[Z(x^n)]}{p^n_X(x^n)}  \leq  \cfrac{(1-\epsilon)}{p_X^n(x^n)} \sum_{w^n \in T_{\delta}(W|x^n)}\tilde{p}_W^n(w^n) p^n_{X|W}(x^n|w^n) \leq  \cfrac{1}{p_X^n(x^n)} \sum_{w^n} p^n_{X,W}(x^n,w^n) =1 \nonumber
\end{align}
where the last inequality above is obtained by adding more terms in the summation and using the definition of $\tilde{p}_W^n(w^n)$ from (\ref{eq:prunedDistribution}).
This simplifies the above probability term as
\begin{align}
    \PP\left(\sum_{l =1}^{2^{n\tilde{R}}}  E^{(\mu_1)}_{L|X^n}(l|x^n) \leq 1\right)  \geq 1 - 2\exp{\bigg(-\cfrac{\eta^2 2^{n(\tilde{R} - I(X,W)-4\delta_1)} }{4 \ln{2}}\bigg)} \nonumber
\end{align}

Using union bound, we extend the above probability to the intersection of all $\mu \in [2^{nC}]$ and $x^n \in T_{\delta}(X)$ 
\begin{align}
\PP\left[\bigcap_{\mu=1}^{2^{nC}}\bigcap_{x^n\in T_{\delta(X)}}\left(\sum_{l =1}^{2^{n\tilde{R}}}  E^{(\mu_1)}_{L|X^n}(l|x^n)\right) \leq 1\right] &\geq 1-\sum_{\mu=1}^{2^{nC}}\sum_{x^n \in T_{\delta}(X)} \PP\left(\sum_{l =1}^{2^{n\tilde{R}}}  E^{(\mu_1)}_{L|X^n}(l|x^n) \leq 1\right) \nonumber\\
&\geq 1 - 2^{nC}|T_{\delta}(X)|2\exp{\bigg(-\cfrac{\eta^2 2^{n(\tilde{R} - I(X,W)-4\delta_1)} }{4 \ln{2}}\bigg)} \label{eq:unionProb}
\end{align}

Therefore, if $\tilde{R} > I(X;W) + 4\delta_1$, the second term in the right hand side of (\ref{eq:unionProb}) decays exponentially to zero and as a result the probability of the above intersections goes to 1.
% This gives for all $x^n \in T_{\delta}(X)$  and $\mu \in [1,2^{nC}]$.
% \begin{align*}
%     \sum_{l =1}^{2^{n\tilde{R}}}  E^{(\mu_1)}_{L|X^n}(l|x^n) &=\cfrac{1}{(1+\eta)} \cfrac{1}{p_{X}^n(x^n)}\left( \cfrac{1}{2^{n\tilde{R}}}\sum_{l =1}^{2^{n\tilde{R}}}Z_l^{(\mu_1)}(x^n)\right) \nonumber \\
%     % \nonumber \\ & \left(\cfrac{1-\epsilon}{1+\eta}\right) \sum_{w^n \in T_{\delta}(W|x^n)} \frac{1}{N}\sum_{l=1}^{N} \mathbbm{1}_{\{W^n(l,\mu_1) = w^n\}} \cfrac{Q^n_{X|W}(x^n|w^n)}{Q^n_X(x^n)} \\
%     %   \cfrac{1}{p_X^n(x^n)}\frac{1}{N}\sum_{l=1}^{N} \left(\cfrac{1-\epsilon}{1+\eta}\right)  Z^{(\mu_1)}_l(x^n) \\
%       &\leq  \left(\cfrac{1-\epsilon}{1+\eta}\right)\cfrac{1}{p_X^n(x^n)}(1+ \eta) \EE[Z(x^n)]  \\
%       & \leq  \cfrac{(1-\epsilon)}{p_X^n(x^n)} \sum_{w^n \in T_{\delta}(W|x^n)}\tilde{p}_W^n(w^n) p^n_{X|W}(x^n|w^n)\\
%      &  \leq  \cfrac{1}{p_X^n(x^n)} \sum_{w^n} p^n_{X,W}(x^n,w^n) =1 \text{ with high probability}
% \end{align*}
% % where the equality uses the definition of $Z^{(\mu_1)}_l(x^n)$ from Eqn. (\ref{def:ZtZ}) and the inequality follows with high probability from (\ref{eq:chernoff1_Z}). Further simplifying the expectation as in Eqn. (\ref{eq:con1}) gives
% % \begin{align}\label{eq:ESmall}
% %     \sum_{w^n \in \{W \backslash w_0\}} E^{(\mu)}_{W^n|X^n}(w^n|x^n) & \leq  \cfrac{(1-\epsilon)}{Q_X^n(x^n)} \sum_{w^n \in T_{\delta}(W|x^n)}\tilde{P}_W^n(w^n) Q^n_{X|W}(x^n|w^n)\\
% %      &  \leq  \cfrac{1}{Q_X^n(x^n)} \sum_{w^n} Q^n_{X,W}(x^n,w^n) =1 \text{ with high probability}.
% % \end{align}
% % where the inequality is obtained by adding more terms in the summation.
% % and using the definition of $\tilde{P}_W^n(w^n)$ from Eqn. (\ref{def:tPw}).
% % where the last inequality above is obtained by adding more terms in the summation and using the definition of $\tilde{p}_W^n(w^n)$ from (\ref{eq:}).
This completes the proof of the lemma.
\end{proof}



% \begin{lemma}\label{lem:conditionSoftCovering}
% \begin{align}
%     \EE\bigg[\sum_{y^n}&|\cfrac{1}{2^{nR}}\sum_{x^n \in T_{\delta}(X)}\sum_{l=1}^{2^{nR}}
%     \mathbbm{1}_{\{X^n(l) = x^n\}} 
%      p^n_{Y|X}(y^n|x^n) - \nonumber \\
%     &\cfrac{1}{2^{nR}}\sum_{x^n\in T_{\delta}(X|y^n)}\sum_{l=1}^{2^{nR}}
%     \mathbbm{1}_{\{X^n(l) = x^n\}} 
%      p^n_{Y|X}(y^n|x^n)|\bigg] \leq \epsilon'
% \end{align}
% where $ T_{\delta}(X|y^n)$ is a $\delta$ conditional typical set of $X$ given $y^n$.
% \end{lemma}
% %  Below, we provide a brief proof to the above required result, the achievability proof later considers the above in detail.
% \begin{proof}
% The left hand side is simply bounded above using typicality as
% % Consider
% % \begin{align}
% %     \sum_{y^n}&|p^n_Y(y^n) - \cfrac{1}{2^{nR}}\sum_{x^n\in T_{\delta}(X|y^n)}\sum_{l=1}^{2^{nR}}
% %     \mathbbm{1}_{\{X^n(l) = x^n\}} 
% %      p^n_{Y|X}(y^n|x^n)|
% %     \nonumber \\
% %     \hspace{-10pt}\leq & \sum_{y^n}|p^n_Y(y^n) - \cfrac{1}{2^{nR}}\sum_{x^n \in T_{\delta}(X)}\sum_{l=1}^{2^{nR}}
% %     \mathbbm{1}_{\{X^n(l) = x^n\}} 
% %      p^n_{Y|X}(y^n|x^n)| \nonumber \\
% %      & +  \sum_{y^n}|\cfrac{1}{2^{nR}}\sum_{x^n \in T_{\delta}(X)}\sum_{l=1}^{2^{nR}}
% %     \mathbbm{1}_{\{X^n(l) = x^n\}} 
% %      p^n_{Y|X}(y^n|x^n)  \nonumber \\ 
% %      & \hspace{30pt}- \cfrac{1}{2^{nR}}\sum_{x^n\in T_{\delta}(X|y^n)}\sum_{l=1}^{2^{nR}}
% %     \mathbbm{1}_{\{X^n(l) = x^n\}} 
% %      p^n_{Y|X}(y^n|x^n)| \nonumber 
% % \end{align}
% % Applying expectation gives
% \begin{align} 
%      &  = \EE\bigg[\sum_{y^n}| \cfrac{1}{2^{nR}}\sum_{x^n\notin T_{\delta}(X|y^n)}\sum_{l=1}^{2^{nR}}
%     \mathbbm{1}_{\{X^n(l) = x^n\}} 
%      p^n_{Y|X}(y^n|x^n)|\bigg]
%      \nonumber \\
%      & = \sum_{y^n} \sum_{x^n\notin T_{\delta}(X|y^n)}p^n_X(x^n) 
%      p^n_{Y|X}(y^n|x^n) \leq \epsilon' \nonumber
% \end{align}
% \end{proof}

\newpage
\bibliographystyle{IEEEtran}
\bibliography{SoftCovering}

==> sideInformation.tex <==
In this section, we provide a characterization of $\mathcal{R}_s(p_{XYZ})$.
\begin{theorem}
\label{Thm:p2pStructured}
$(R,C) \in \mathcal{R}(p_{XY})$ if and only if there exists a PMF $p_{WXY}$ such that (i) $p_{XY}(x,y) = \sum_{w \in \mathcal{W}}p_{WXY}(w,x,y)$ for all $(x,y)$ where $\mathcal{W}$ is the alphabet of $W$, (ii) $X-W-Y$ is a Markov chain, (iii) $|\mathcal{W}| \leq ( |\mathcal{X}||\mathcal{Y}|)^2$, and 
 $R \geq I(X;W),  R+C \geq I(XY;W).$
\end{theorem}
\begin{proof} We provide the main elements (achievability in Sec.~\ref{SubSec:p2pAchievability} and converse in Sec.~\ref{SubSec:p2pConverse}) of our proof here with particular emphasis on the new elements. The reader is referred to \cite{arxiv_CurrentPaper} for more technical details.
\vspace{-0.15cm}

\subsection{Achievability}
\label{SubSec:p2pAchievability}


\subsection{Converse}
\label{SubSec:SideInfoConverse}
The proof for the converse is provided in \cite{CuffPhDThesis}.
\end{proof}
